On the Generalization of Wasserstein Robust Federated Learning

In federated learning, participating clients typically possess non-i.i.d. data, posing a significant challenge to generalization to unseen distributions. To address this, we propose a Wasserstein distributionally robust optimization scheme called WAFL. Leveraging its duality, we frame WAFL as an empirical surrogate risk minimization problem, and solve it using a local SGD-based algorithm with convergence guarantees. We show that the robustness of WAFL is more general than related approaches, and the generalization bound is robust to all adversarial distributions inside the Wasserstein ball (ambiguity set). Since the center location and radius of the Wasserstein ball can be suitably modified, WAFL shows its applicability not only in robustness but also in domain adaptation. Through empirical evaluation, we demonstrate that WAFL generalizes better than the vanilla FedAvg in non-i.i.d. settings, and is more robust than other related methods in distribution shift settings. Further, using benchmark datasets we show that WAFL is capable of generalizing to unseen target domains.

==> neurips_sections/convergence_with_approx_tmp.tex <==
The design of \OurAlg leads to an empirical surrogate risk minimization problem. Given model parameters $\theta$ and training example $z_i$, the original loss function is $\ell(z_i, \theta)$. \OurAlg then finds the adversarial example corresponding to $z_i$, by solving the following
\begin{align*}
	\max_{\zeta} \BigC{\varphi_\gamma(\zeta, \theta; z_i) \defeq \ell(\zeta, \theta) - \gamma d^2(\zeta, z_i)}.
\end{align*}
Let $z_i^*$ be the solution to this problem, and $\phi_\gamma(z_i, \theta) = \varphi_\gamma(z_i^*, \theta; z_i)$. Let \Cref{Assumption:smooth_loss} hold and assume that \blue{$d$ is $1$-strongly convex in its first argument} and $\gamma > L_{zz}$. Then $\varphi_\gamma(\zeta, \theta; z_i)$ is $(\gamma - L_{zz})$-strongly concave with respect to $\zeta$. This makes the above optimization problem easy with linear convergence guarantee using gradient ascent. Instead of solving for $z_i^*$ exactly, we approximate it using \blue{gradient ascent} until a solution $\widehat{z}_i$ is found satisfying the condition
\begin{align*}
	\norm{\widehat{z}_i - z_i^*} \leq \delta.
\end{align*}
Because $\varphi_\gamma(\zeta, \theta; z_i)$ is smooth and strongly concave with respect to $\zeta$, such a solution $\widehat{z}_i$ can be found in $O(\log(1/\delta))$ iterations.

% Fix some $z_i$. Define $\varphi(\zeta, \theta; z_i) \defeq \ell(\zeta, h_\theta) - \gamma d(\zeta, z_i).$  Since $\ell$ is $L_{zz}$-smooth and $d$ is $1$-strongly convex, $\varphi(\zeta, \theta; z_i)$ is $(\gamma - L_{zz})$-strongly concave with respect to $\zeta$, given that $\gamma > L_{zz}$.

\subsection{Smoothness of $\phi_\gamma$} \label{appn:smooth_phi_gamma}

\blue{To simplify notation, hereinafter we use the $\nabla$ notation to denote the gradient of a function \emph{with respect to $\theta$}}. \citet[Lemma 1]{sinha_certifying_2020} show that that the surrogate loss $\phi_\gamma$ is smooth with respect to $\theta$. We summarize that in the following lemma.

\begin{lemma} \label{Lemma:f_smooth}
	Let $z_i^* = \argmax_{\zeta \in \mathcal{Z}}\varphi(\zeta, \theta; z_i)$. \blue{Therefore, $\phi_{\gamma}(\theta; z_i) = \varphi_\gamma(z_i^*, \theta; z_i).$} Let $\ell$ satisfy Assumption \ref{Assumption:smooth_loss}. Then $\phi_{\gamma}$ is differentiable, and
	\begin{align*}
		\norm{\nabla \phi_{\gamma}(z_i, \theta) - \nabla \phi_{\gamma}(z_i, \theta')} \leq L \norm{\theta - \theta'},
	\end{align*}
	with $L = L_{\theta \theta} + \frac{L_{\theta z} L_{z \theta}}{\gamma - L_{zz}}$ when $\gamma > L_{zz}$.
\end{lemma}

\subsection{Variance of stochastic gradients}

Define $g_{i}(\theta) \defeq \frac{1}{\abs{\gD_i}} \SumNoLim{z_i \in \gD_i}{}\nabla \phi_{\gamma} ({z}_i, \theta)$. Then we have 
\begin{align} \label{E:bounded_var}
	&\mathbf{E}\BigS{\norm{g_i(\theta) - \nabla F_i(\theta)}^2} =  \mathbf{E} \BigS{\BigNorm{ \frac{1}{\abs{\gD_i}} \SumLim{z_i \in \gD_i}{}\nabla \phi_{\gamma}({z}_i, {\theta}) - \nabla F_i(\theta)}^2} \nonumber\\
	&\leq  \frac{1}{\abs{\gD_i}}  \mathbf{E} \BigS{\bigNorm{  g_{\phi_i}( {\theta}) - \nabla F_i(\theta)}^2} 
	 \leq \frac{\sigma^2}{\abs{\gD_i}} \defeq \widehat{\sigma}^2.  \quad \text{ (by \Cref{Assumption:bounded_variance}.)   }
\end{align}

\subsection{Further properties involving approximate adversarial solution $\widehat{z}_i$}

We now establish some further properties of $\phi_\gamma$ relating to this approximate solution. First, we have \blue{(noting that the gradients below are with respect to $\theta$)}
\begin{align*}
	\norm{\nabla \phi_\gamma(z_i, \theta) - \nabla \varphi_\gamma(\widehat{z}_i, \theta; z_i)} & = \norm{\nabla \varphi_\gamma(z_i^*, \theta; z_i) - \nabla \varphi_\gamma(\widehat{z}_i, \theta; z_i)} \\
	& = \norm{\nabla \ell(z_i^*, \theta) - \nabla \ell(\widehat{z}_i, \theta)} \\
	& \leq L_{\theta z} \norm{z_i^* - \widehat{z}_i} ~~~~ \text{(By \Cref{Assumption:smooth_loss})} \\
	& \leq L_{\theta z} \delta.
\end{align*}
This shows that, approximating the surrogate gradient $\nabla_{\theta} \phi_{\gamma} (z_i, \theta)$ using $\widehat{z}_i$ incurs an error of $L_{\theta z} \delta$.

% Using similar notation as in \cite{wang_field_2021}, 
% define $g_i(\theta) = \nabla \phi_\gamma(z_i, \theta)$, and  Therefore, we have
\blue{Define $\tilde{g}_i(\theta) \defeq \frac{1}{\abs{\gD_i}} \SumNoLim{z_i \in \gD_i}{} \nabla \varphi_\gamma(\widehat{z_i}, \theta; z_i)$. This quantity represents the approximation to the stochastic gradient $g_i(\theta)$ using approximately-solved adversarial examples $\widehat{z}_i$. Therefore,
\begin{align*}
	\norm{\tilde{g}_i(\theta) - g_i(\theta)} & = \BigNorm{\frac{1}{\abs{\gD_i}} \SumNoLim{z_i \in \gD_i}{} \bigS{\nabla \varphi_\gamma(\widehat{z}_i, \theta; z_i)} - \nabla \phi_\gamma(z_i, \theta)} \\
	& \leq \frac{1}{\abs{\gD_i}} \SumNoLim{z_i \in \gD_i}{} \BigNorm{ \nabla \varphi_\gamma(\widehat{z}_i, \theta; z_i) - \nabla \phi_\gamma(z_i, \theta)} \\
	& \leq L_{\theta z} \delta.
\end{align*}
}

\subsection{Convergence proof}

Our proof is based on the analysis of local SGD for FL presented by \citet[Theorem 1]{wang_field_2021}. First, define the ``shadow sequence'' as
\begin{align*}
    \bar{\theta}^{(t, k)} = \SumNoLim{i=1}{m} \lambda_i \theta_i^{(t, k)}.
\end{align*}
We therefore have
\blue{
\begin{align*}
	\bar{\theta}^{(t, k+1)} 
	= \SumLim{i=1}{m} \lambda_i \theta_i^{(t, k+1)} 
	= \SumLim{i=1}{m} \lambda_i \bigP{\theta_i^{(t, k)} - \eta \tilde{g}_i(\theta_i^{(t, k)})} 
	= \bar{\theta}^{(t, k)} - 
	\eta
	\SumLim{i=1}{m}
	\lambda_i \tilde{g}_i(\theta_i^{(t, k)}).
\end{align*}
}

The proof is based on two following intermediate results. \cref{lem:progress} bounds the progress made at every global round and \cref{lem:bounded_client_drift} bounds the client drift, which is the difference between the local parameters and shadow sequence.

\begin{lemma} \label{lem:progress}
	Assuming the local learning rate satisfies $\eta \leq \frac{1}{4L}$, then
	\begin{align*}
		\mathbf{E}\BiggS{\frac{1}{K} \SumLim{k=1}{K} F(\bar{\theta}^{(t, k)}) - F(\theta^*)} & \leq \frac{1}{4 \eta K} \BigP{\norm{\bar{\theta}^{(t, 0)} - \theta^*}^2 - \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, K)} -\theta^*}^2}} \\
		& ~~~~~ + \eta \widehat{\sigma}^2 \Lambda + \eta L_{\theta z}^2 \delta^2 + \frac{L}{K} \SumLim{i=1}{m} \lambda_i \SumLim{k=0}{K-1} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2}.
	\end{align*}
\end{lemma}

\begin{proof}
	Since $F_i$ is $L$-Lipschitz smooth \blue{(\Cref{Lemma:f_smooth})},
	\begin{align*}
		F_i(\bar{\theta}^{(t, k+1)}) & \leq F_i(\theta_i^{(t, k)}) + \innProd{\nabla F_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta_i^{(t, k)}} + \frac{L}{2} \norm{\bar{\theta}^{(t, k+1)} - \theta_i^{(t, k)}}^2 \\
		& \leq F_i(\theta^*) + \innProd{\nabla F_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*} + \frac{L}{2} \norm{\bar{\theta}^{(t, k+1)} - \theta_i^{(t, k)}}^2 ~~~~~ \text{($F_i$ is convex)}\\ 
		& \leq F_i(\theta^*) + \innProd{\nabla F_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*} + L \norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2 + L \norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2.
	\end{align*}
	Therefore,
	\begin{align*}
		F_i(\bar{\theta}^{(t, k+1)}) - F_i(\theta^*) \leq \innProd{\nabla F_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*} + L \norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2 + L \norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2.
	\end{align*}
	Taking the weighted average among all clients:
	\begin{align}
		F(\bar{\theta}^{(t, k+1)}) - F(\theta^*) & = \SumLim{i=1}{m} \lambda_i \bigS{F_i(\bar{\theta}^{(t, k+1)}) - F_i(\theta^*)} \nonumber \\
		& \leq \SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*} + L \norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2 \nonumber \\
		& ~~~~~ + L \SumLim{i=1}{m} \lambda_i \norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2 \nonumber \\
		& \leq \SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}) - \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*} + L \norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2 \nonumber \\
		& ~~~~~ + L \SumLim{i=1}{m} \lambda_i \norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2 + \SumLim{i=1}{m} \lambda_i \innProd{ \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*}. \label{E:bound_1}
	\end{align}
	First, we bound the expectation of the fourth term the fourth term of \cref{E:bound_1} by using the parallelogram law:
	\begin{align}
		& \mathbf{E}\BiggS{\SumLim{i=1}{m} \lambda_i \innProd{ \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*}}  = \mathbf{E}\BiggS{\frac{1}{\eta} \innProd{\bar{\theta}^{(t, k)} - \bar{\theta}^{(t, k+1)}, \bar{\theta}^{(t, k+1)} - \theta^*}} \nonumber \\
		= & \frac{1}{2\eta} \BigP{\norm{ \bar{\theta}^{(t, k)} - \theta^*}^2 - \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} - \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}} \nonumber \\
% 		& \leq \frac{1}{2\eta} \BigP{\norm{ \bar{\theta}^{(t, k)} - \theta^*}^2 - \mathbf{E}\bigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}} - \blue{\frac{1}{4 \eta}} 	\mathbf{E}\bigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} \label{E:bound_2} \\
		= & \blue{\frac{1}{2 \eta}  \norm{ \bar{\theta}^{(t, k)} - \theta^*}^2 - \frac{1}{2 \eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} - \frac{1}{2 \eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}}. \label{E:bound_2}
	\end{align}
	Now we bound the first term of \cref{E:bound_1} as follows
	\begin{align} \label{E:X}
		& \SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}) - \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*} \nonumber \\
		= &  \underbrace{\SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}) - g_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*}}_\text{$A$} + \SumLim{i=1}{m} \lambda_i \underbrace{\innProd{g_i(\theta_i^{(t, k)}) - \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*}}_\text{$B$}.
	\end{align}
	Because $g_i$ is an unbiased estimate of $\nabla F_i$ with variance bounded by $\widehat{\sigma}^2$ \blue{(by \Cref{Assumption:bounded_variance,E:bounded_var})}, we bound the expectation of $A$ as follows:
	\blue{
	\begin{align}
		\mathbf{E}\bigS{A} & = \mathbb{E} \BiggS{\SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}) - g_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \bar{\theta}^*}} \nonumber \\
		& = \mathbb{E} \BiggS{\SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}) - g_i(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}} \nonumber \\
		& \leq \eta \mathbf{E} \BiggS{\BigNorm{\SumLim{i=1}{m} \lambda_i \bigP{\nabla F_i(\theta_i^{(t, k)}) - g_i(\theta_i^{(t, k)})}}^2} + \frac{1}{4 \eta}  \mathbf{E} \BigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} \quad \text{(by Young's inequality)} \nonumber \\
		& \leq \eta \widehat{\sigma}^2 \Lambda + \frac{1}{4\eta} \mathbf{E} \BigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2}. \label{E:E_A}
	\end{align}
	}
	Now we bound the expectation of $B$ as follows:  % \blue{with $\epsilon = \frac{1}{2\eta}$}
	\begin{align}
		\mathbf{E}\bigS{B} &= \mathbf{E}\BigS{\innProd{g_i(\theta_i^{(t, k)}) - \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*}} \nonumber \\
		& \blue{\leq \eta \mathbf{E}\BigS{\norm{g_i(\theta_i^{(t, k)}) - \tilde{g_i}(\theta_i^{(t, k)})}^2} + \frac{1}{4\eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2} \quad \text{(by Young's inequality)}} \nonumber \\
		& \blue{\leq \eta L_{\theta z}^2 \delta^2 + \frac{1}{4\eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}.} \label{E:E_B}
	\end{align}
	Taking the expectation on both sides of \Cref{E:X} and substituting \Cref{E:E_A} and \Cref{E:E_B} to the right-hand side gives
	\begin{align}
		& \mathbf{E}\BiggS{\SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}) - \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*}} \nonumber \\
		\leq & \eta \widehat{\sigma}^2 \Lambda + \frac{1}{4\eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} + \blue{\eta L_{\theta z}^2 \delta^2 + \frac{1}{4\eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}}. \label{E:bound_3}
	\end{align}
	Taking the expectation on both sides of \cref{E:bound_1} and substituting \cref{E:bound_2} and \cref{E:bound_3} to the right-hand side gives
	\begin{align*}
		\mathbf{E}\BigS{F(\bar{\theta}^{(t, k+1)}) - F(\theta^*)} &\leq \eta \widehat{\sigma}^2 \Lambda + \frac{1}{4\eta} \mathbf{E}\bigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} + \eta L_{\theta z}^2 \delta^2 \blue{+ \frac{1}{4\eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}} \\
		& ~~~~~ + L \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} + L \SumLim{i=1}{m} \lambda_i \norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2 \\
% 		& ~~~~~ + \frac{1}{2\eta} \BigP{\norm{ \bar{\theta}^{(t, k)} - \theta^*}^2 - \mathbf{E}\bigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}} - \blue{\frac{1}{2 \eta}} 	\mathbf{E}\bigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} \\
        & ~~~~~ \blue{+ \frac{1}{2 \eta} \norm{ \bar{\theta}^{(t, k)} - \theta^*}^2 - \frac{1}{2 \eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2}} - \frac{1}{2 \eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} \\
		& \leq \eta \widehat{\sigma}^2 \Lambda + \eta L_{\theta z}^2 \delta^2 - \BigP{\frac{1}{4\eta} - L} \mathbf{E}\bigS{\norm{\bar{\theta}^{(t, k+1)} - \bar{\theta}^{(t, k)}}^2} \\
		& ~~~~~ + L \SumLim{i=1}{m} \lambda_i \norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2 \\
		& ~~~~~ \blue{- \frac{1}{4\eta} \norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2 + \frac{1}{2\eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k)} - \theta^*}^2}} \\
		& \leq \eta \widehat{\sigma}^2 \Lambda + \eta L_{\theta z}^2 \delta^2 + L \SumLim{i=1}{m} \lambda_i \norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2 \\
		& ~~~~~ \blue{- \frac{1}{4\eta} \norm{\bar{\theta}^{(t, k+1)} - \theta^*}^2 + \frac{1}{2\eta} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k)} - \theta^*}^2}}. \quad \text{(Since $\eta \leq 1/4L$)}
	\end{align*}
	Telescoping $k$ from $0$ to $K-1$:
	\begin{align*}
		\mathbf{E}\BiggS{\frac{1}{K} \SumLim{k=1}{K} F(\bar{\theta}^{(t, k)}) - F(\theta^*)} & \leq \blue{\frac{1}{4 \eta K}} \BigP{\norm{\bar{\theta}^{(t, 0)} - \theta^*}^2 - \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, K)} -\theta^*}^2}} \\
		& ~~~~~ + \eta \widehat{\sigma}^2 \Lambda + \eta L_{\theta z}^2 \delta^2 + \frac{L}{K} \SumLim{i=1}{m} \lambda_i \SumLim{k=0}{K-1} \mathbf{E}\BigS{\norm{\bar{\theta}^{(t, k)} - \theta_i^{(t, k)}}^2}.
	\end{align*}
\end{proof}

\begin{lemma} \label{lem:bounded_client_drift}
	Assuming the client learning rate satisfies $\eta \leq  \frac{1}{3L}$, we have
	\begin{align*}
		\mathbf{E}\BigS{\norm{\theta_i^{(t, k)} - \bar{\theta}^{(t, k)}}^2} \leq  \eta^2( 24 K^2 \bar{\Omega}^2 + 20 K \bar{\Omega}^2). 
	\end{align*}
where $\bar{\Omega}^2 \defeq \max\bigC{\widehat{\sigma}^2 , \Omega^2}$. 
\end{lemma}

\begin{proof}	
\begin{align}
	\mathbf{E} & \biggS{\bigNorm{\theta_{1}^{(t, k+1)} - \theta_{2}^{(t, k+1)}}^2} = \mathbf{E}\biggS{\BigNorm{\theta_{1}^{(t, k)} - \theta_{2}^{(t, k)} - \eta\BigP{g_{1}(\theta_{1}^{(t, k)}) -  g_{2}(\theta_{1}^{(t, k)})}}^2} \nonumber \\
	= & \norm{\theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}}^2 - 2 \eta \innProd{g_{1}(\theta_{1}^{(t, k)}) - \nabla F_{1}(\theta_1^{(t,k)}), \theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}} \nonumber \\
	& - 2 \eta \innProd{\nabla F_{2}(\theta_1^{(t,k)})- g_{2}(\theta_{2}^{(t, k)}), \theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}} \nonumber\\
	&- 2 \eta \innProd{\nabla F_{1}(\theta_1^{(t,k)}) - \nabla F_{2}(\theta_2^{(t,k)}), \theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}} +\eta^2 \norm{g_{1}(\theta_{1}^{(t, k)}) - g_{2}(\theta_{2}^{(t, k)})}^2.  \label{E:localrounds}
\end{align}
The second term (and similarly for the third term)  is bounded as follows
\begin{align*}
- &\innProd{g_{1}(\theta_{1}^{(t, k)}) - \nabla F_{1}(\theta_1^{(t,k)}), \theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}} \\
&\leq  \frac{1}{6 \eta K}  \bigNorm{\theta_1^{(t,k)} - \theta_2^{(t,k)}}^2 + \frac{3 \eta K}{2} \bigNorm{g_{1}(\theta_{1}^{(t, k)}) - \nabla F_{1}(\theta_1^{(t,k)})}^2 \quad & \text{(by Young's inequality)}\\
& = \frac{1}{6 \eta K}  \bigNorm{\theta_1^{(t,k)} - \theta_2^{(t,k)}}^2 + \frac{3 \eta K}{2} \widehat{\sigma}^2    \qquad\text{(by \Cref{E:bounded_var})}
\end{align*}
Since $\max_{i} \sup_{\theta} \norm{\nabla F_i(\theta) - \nabla F(\theta)} \leq \Omega$ (\Cref{Assumption:bounded_gradient_surrogate}), the fourth term is bounded as
\begin{align*}
	&-\innProd{\nabla F_{1}(\theta_1^{(t,k)}) - \nabla F_{2}(\theta_2^{(t,k)}), \theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}}\\
	\leq & -\innProd{\nabla F(\theta_1^{(t,k)}) - \nabla F(\theta_2^{(t,k)}), \theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}} + 2 \Omega \norm{\theta_1^{(t,k)} - \theta_2^{(t,k)}}\\
	\leq & -\frac{1}{L} \norm{\nabla F(\theta_1^{(t,k)}) - \nabla F(\theta_2^{(t,k)})}^2 + 2 \Omega \norm{\theta_1^{(t,k)} - \theta_2^{(t,k)}} &\text{(by smoothness and convexity)}\\
	\leq & -\frac{1}{L} \norm{\nabla F(\theta_1^{(t,k)}) - \nabla F(\theta_2^{(t,k)})}^2 + \frac{1}{6 \eta K} \norm{\theta_1^{(t,k)} - \theta_2^{(t,k)}}^2 + 6 \eta K \Omega^2 &\text{(by Young's inequality)}
\end{align*}

The last term is bounded as follows
\begin{align*}
&\norm{g_{1} (\theta_{1}^{(t, k)}) - g_{2}(\theta_{2}^{(t, k)})}^2  \\
&\leq 5 \BigP{\bigNorm{g_{1}(\theta_{1}^{(t, k)}) - \nabla F_{1}(\theta_1^{(t,k)})}^2 +
	\norm{\nabla F_{1}(\theta_1^{(t,k)}) - \nabla F(\theta_1^{(t,k)})}^2  + \norm{\nabla F(\theta_1^{(t,k)}) - \nabla F (\theta_2^{(t,k)})}^2 \\
	& \quad + \norm{\nabla F(\theta_2^{(t,k)}) - \nabla F_{2}(\theta_2^{(t,k)})}^2 + \bigNorm{g_{2}(\theta_{2}^{(t, k)}) - \nabla F_{2}(\theta_2^{(t,k)})}^2} \\
& \leq 5 \norm{\nabla F(\theta_1^{(t,k)}) - \nabla F(\theta_2^{(t,k)})}^2 + 10 (\widehat{\sigma}^2 + \Omega^2) \quad \text{(by \Cref{E:bounded_var} and \Cref{Assumption:bounded_gradient_surrogate})}
\end{align*}


Substituting the above four bounds back to \cref{E:localrounds} gives (note that $\eta \leq \frac{1}{3L}$)
\begin{align*}
	\mathbf{E}&\BigS{\norm{\theta_{1}^{(t, k+1)} - \theta_{2}^{(t, k+1)}}^2} \leq \BigP{1 + \frac{1}{K}} \norm{\theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}}^2 - \eta \BigP{\frac{2}{L} - 5 \eta} \bigNorm{\nabla F(\theta_1^{(t,k)}) - \nabla F(\theta_2^{(t,k)})}^2 \\
	& \quad + 6 \eta^2 K \widehat{\sigma}^2 + 12  \eta^2 K \Omega^2 + 10 \eta^2 (\widehat{\sigma}^2 + \Omega^2)  \\
	& \leq \BigP{1 + \frac{1}{K}} \norm{\theta_{1}^{(t, k)} - \theta_{2}^{(t, k)}}^2 + 6 \eta^2 K \widehat{\sigma}^2 + 12  \eta^2 K \Omega^2 + 10 \eta^2 (\widehat{\sigma}^2 + \Omega^2).
\end{align*}

Unrolling recursively, we obtain
\begin{align*}
	\mathbf{E}\BigS{\bigNorm{\theta_{1}^{(t, k+1)} - \theta_{2}^{(t, k+1)}}^2} &\leq \frac{\bigP{1 + {1}/{K}}^K - 1}{{1}/{K}}  \BigS{ 6 \eta^2 K \widehat{\sigma}^2 + 12  \eta^2 K \Omega^2 + 10 \eta^2 (\widehat{\sigma}^2 + \Omega^2)}  \\
	&\leq  12 \eta^2 K^2 \widehat{\sigma}^2 + 24 \eta^2 K^2 \Omega^2 + 20 \eta^2 K (\widehat{\sigma}^2 + \Omega^2)\\
	&\leq  \eta^2( 24 K^2 \bar{\Omega}^2 + 20 K \bar{\Omega}^2). 
\end{align*}
where we use the fact that $\frac{\bigP{1 + {1}/{K}}^K - 1}{{1}/{K}} \leq K (e - 1) \leq 2K$, and $\bar{\Omega}^2 \defeq \max\bigC{\widehat{\sigma}^2 , \Omega^2}$. 

By convexity, for any $i$,
\begin{align*}
\mathbf{E}\BigS{\norm{\theta_{i}^{(t, k+1)} - \bar{\theta}^{(t, k+1)}}^2} 
%&\leq 12 \eta^2 K^2 \widehat{\sigma}^2 + 24 \eta^2 K^2 \Omega^2 + 20 \eta^2 K (\widehat{\sigma}^2 + \Omega^2). \\
\leq  \eta^2( 24 K^2 \bar{\Omega}^2 + 20 K \bar{\Omega}^2). 
\end{align*}
\end{proof}

\blue{TODO: OPTIMIZE $\eta$ on the RHS

Substituting the result of \Cref{lem:bounded_client_drift} to \Cref{lem:progress}, and telescoping over $t$, we obtain
\begin{align*}
	\mathbb{E}\BiggS{\frac{1}{T} \SumLim{t=0}{T-1} \frac{1}{K} \SumLim{k=1}{K} F(\bar{\theta}^{(t, k)}) - F({\theta}^*)} 
	\leq  & \frac{D^2}{4 \eta K T}
	+ \eta \widehat{\sigma}^2 \Lambda + \eta L_{\theta z}^2 \delta^2  + \eta^2 L ( 24 K^2 \bar{\Omega}^2 + 20 K \bar{\Omega}^2), 
\end{align*}

where $D \defeq \norm{\theta^{(0)} - {\theta}^*}$,  $ \Lambda \defeq {\SumLim{i=1}{m} \lambda_i^2}$. By optimizing $\eta$ on the R.H.S., we obtain
\begin{align*}
\mathbb{E}\BigS{\frac{1}{KT} \SumLim{t=0}{T-1} \SumLim{k=1}{K}  F(\bar{\theta}^{(t, k)}) - F({\theta}^*)} 
\leq  \gO \biggP{{\frac{ L D^2}{KT} + 
	\frac{ \widehat{\sigma} D \Lambda^{\frac{1}{2}}}{\sqrt{ KT}}} + 
{\frac{ L^{\frac{1}{3}} \bar{\Omega}^{\frac{2}{3}} D^{\frac{4}{3}}}{K^{\frac{1}{3}} T^{\frac{2}{3}}} + 
	\frac{ L^{\frac{1}{3}} \bar{\Omega}^{\frac{2}{3}} D^{\frac{4}{3}}}{T^{\frac{2}{3}}}}},
\end{align*}
when 
\begin{align*}
\eta = \min{\set{\frac{1}{3L}, \frac{ D}{2 \sqrt{ K T\Lambda} \widehat{\sigma}}, \frac{D^{\frac{2}{3}}}{48^{\frac{1}{3}}K^{\frac{2}{3}} T^{\frac{1}{3}} L^{\frac{1}{3}} \bar{\Omega}^{\frac{2}{3}}}, \frac{D^{\frac{2}{3}}}{40^{\frac{1}{3}} K T^{\frac{1}{3}} L^{\frac{1}{3}} \bar{\Omega}^{\frac{2}{3}}}}}. 
\end{align*}

\textcolor{red}{
	Now we bound the first term of \cref{E:bound_1} as follows
	\begin{align} \label{TA_E:X}
		& \SumLim{i=1}{m} \lambda_i \innProd{\nabla F_i(\theta_i^{(t, k)}) - \tilde{g_i}(\theta_i^{(t, k)}), \bar{\theta}^{(t, k+1)} - \theta^*} \nonumber 
	\end{align}
}

}
